Signed Networks, Triadic Interactions and the Evolution of Cooperation

We outline a model to study the evolution of cooperation in a population of agents playing the prisoner's dilemma in signed networks. We highlight that if only dyadic interactions are taken into account, cooperation never evolves. However, when triadic considerations are introduced, a window of opportunity for emergence of cooperation as a stable behaviour emerges.

==> eptcsdata.tex <==
\providecommand{\firstpage}{104}
\providecommand{\publicationstatus}{A. Graudenzi, G. Caravagna, G. Mauri, M. Antoniotti (Eds.): \\Wivace 2013 - Italian Workshop on \\Artificial Life and Evolutionary Computation\\
EPTCS 130, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.130.17}{10.4204/EPTCS.130.17}}
\pdfoutput=1

